FreeDNA: Endowing Domain Adaptation of Diffusion-Based Dense Prediction with Training-Free Domain Noise Alignment

Domain Adaptation(DA) for dense prediction tasks is an important topic, which enhances the dense prediction model's performance when tested on its unseen domain. Recently, with the development of Diffusion-based Dense Prediction (DDP) models, the exploration of DA designs tailored to this framework is worth exploring, since the diffusion model is effective in modeling the distribution transformation that comprises domain information. In this work, we propose a training-free mechanism for DDP frameworks, endowing them with DA capabilities. Our motivation arises from the observation that the exposure bias (e.g., noise statistics bias) in diffusion brings domain shift, and different domains in conditions of DDP models can also be effectively captured by the noise prediction statistics. Based on this, we propose a training-free Domain Noise Alignment (DNA) approach, which alleviates the variations of noise statistics to domain changes during the diffusion sampling process, thereby achieving domain adaptation. Specifically, when the source domain is available, we directly adopt the DNA method to achieve domain adaptation by aligning the noise statistics of the target domain with those of the source domain. For the more challenging source-free DA, inspired by the observation that regions closer to the source domain exhibit higher confidence meeting variations of sampling noise, we utilize the statistics from the high-confidence regions progressively to guide the noise statistic adjustment during the sampling process. Notably, our method demonstrates the effectiveness of enhancing the DA capability of DDP models across four common dense prediction tasks. Code is available at \href{https://github.com/xuhang07/FreeDNA}{https://github.com/xuhang07/FreeDNA}.

==> sec/sdda.tex <==
\begin{algorithm}[htbp]
\caption{Source-Available Domain Adaptation For Diffusion Model with Domain Noise Alignment}
\label{alg:sdda}
\begin{algorithmic}[1]
\REQUIRE Source domain $D_t$, diffusion model $\epsilon_\theta(x_t,t,c)$, Timestep $t_i$
\ENSURE Output list $n_{all}$
\FOR{each $c_t \in D_t$}
    \STATE sample $x_T \in N(0,1)$, $n_t=()$
    \FOR{each $t = T$ to $0$ step $t_i$}
        \STATE $\epsilon_t = \epsilon_\theta(x_t,c,c_t)$, $n_t.append(\|\epsilon_t\|_2)$
        \STATE $x_{t-1} = scheduler.step(\epsilon_t, t, x_t).prev\_sample$
    \ENDFOR
    \STATE $n_{all}.append(n_t)$
\ENDFOR
\STATE $n_{all} = n_{all}.mean(dim=0)$
\RETURN $n_{all}$
\end{algorithmic}

\begin{algorithmic}[2]
\REQUIRE Target image $c_s$, diffusion model $\epsilon_\theta(x_t,t,c)$, Source domain noise list $n_{all}$, Timestep $t_i$
\ENSURE Output result $x_0$
\STATE Initialize $\delta_0=0$, $\delta_1=0$, $\lambda=1$, $x_T \in N(0,1)$
\FOR{each $t = T$ to $1$ step $t_i$}
    \STATE $\epsilon_t = \epsilon_\theta(x_t,c,c_s)$, $\delta_1 = \|\epsilon_t\|_2 / n_{all}[(T-t)/t_i]$
    \IF {$\delta_0 \neq 0$}
        \STATE $\lambda = \delta_1-\delta_0+1-{sum}_\lambda$
    \ENDIF
    \STATE ${sum}_\lambda = {sum}_\lambda+\lambda-1$, $\delta_0 = \delta_1$
    \STATE $\hat{x_0} = (x_t-\sqrt{\bar{\beta}_t}\epsilon_t/\lambda)/\sqrt{\bar{\alpha}_t}$
    \STATE $x_{t-1} = \sqrt{\bar{\alpha}_{t-1}}\hat{x_0}+(1-\sqrt{\bar{\alpha}_{t-1}})\epsilon_t$
\ENDFOR
\RETURN $x_0$
\end{algorithmic}
\end{algorithm}

==> sec/sfda.tex <==
\begin{algorithm}[htbp]
\caption{Source-Free Domain Adaptation For Diffusion Model with Domain Noise Alignment}
\label{alg:sfda}
\begin{algorithmic}[1]
\REQUIRE Target image $c_s$, diffusion model $\epsilon_\theta(x_t,t,c)$, Timestep $t_i$, Linear mask schedule $P$, Sample times $k$
\ENSURE Output result $x_0$
\STATE Initialize $\delta_0=0$, $\delta_1=0$, $\lambda=1$
\STATE sample $x_{T_1}, \dots, x_{T_k} \in N(0,1)$, 
\FOR{each $t = T$ to $1$ step $t_i$}
    \FOR{each $i = 1$ to $k$}
        \STATE $\epsilon_{t_i} = \epsilon_\theta(x_{t_i},c,c_s)$
        \STATE $\hat{x_{0_i}} = (x_t-\sqrt{\bar{\beta}_t}\epsilon_{t_i}/\lambda)/\sqrt{\bar{\alpha}_t}$
    \ENDFOR
    \STATE $\gamma = cal\_consistency(\epsilon_{t_1},\dots,\epsilon_{t_k}), p_t = P[T/t_i]$
    \STATE $M = quantile(stack[\hat{x_{0_1}},\dots,\hat{x_{0_k}}].var(0),p_t)$
    \STATE $\delta_1 = \|\epsilon_t\|_2 / \|\epsilon_t[M]\|_2$
    \IF {$\delta_0 \neq 0$}
        \STATE $\lambda = (\delta_1-\delta_0+1-{sum}_\lambda)\gamma$
    \ENDIF
    \STATE ${sum}_\lambda = {sum}_\lambda+\lambda-1, \delta_0 = \delta_1$
    \FOR{each $i = 1$ to $k$}
        \STATE $\hat{x_{0_i}} = (x_{t_i}-\sqrt{\bar{\beta}_t}\epsilon_{t_i}/\lambda)/\sqrt{\bar{\alpha}_t}$
        \STATE ${x_{t-1}}_i = \sqrt{\bar{\alpha}_{t-1}}\hat{x_{0_i}}+(1-\sqrt{\bar{\alpha}_{t-1}}){\epsilon_{t_i}}$
    \ENDFOR
\ENDFOR
\RETURN $ensemble(x_{0_1}, \dots, x_{0_k})$
\end{algorithmic}
\end{algorithm}
